Detecting Data Leakage from Databases on Android Apps with Concept Drift

Mobile databases are the statutory backbones of many applications on smartphones, and they store a lot of sensitive information. However, vulnerabilities in the operating system or the app logic can lead to sensitive data leakage by giving the adversaries unauthorized access to the app's database. In this paper, we study such vulnerabilities to define a threat model, and we propose an OS-version independent protection mechanism that app developers can utilize to detect such attacks. To do so, we model the user behavior with the database query workload created by the original apps. Here, we model the drift in behavior by comparing probability distributions of the query workload features over time. We then use this model to determine if the app behavior drift is anomalous. We evaluate our framework on real-world workloads of three different popular Android apps, and we show that our system was able to detect more than 90% of such attacks.

==> Makefile <==
TEX_FILES=paper.tex paperGokhan.bib $(wildcard sections/*)

all: clean paper.pdf todo
	@if [ `uname` = "Darwin" ] ; then open paper.pdf; fi

graphs:
	@cd graphs; rake

paper.pdf: $(TEX_FILES)
	latexmk -pdf paper.tex 

open: paper.pdf todo
	open $<
	
clean:
	latexmk -CA -bibtex

todo:
	@echo "==========================="
	@echo "     Remaining Todos "
	@echo "==========================="
	@find sections -name '*.tex' | \
		xargs grep 'todo' | \
		sed 's:^sections/::; s:\.tex::' | \
		sed 's/\([^:]*\):.*\\todo{/TODO (\1): /; s/}.*//;'


.PHONY: todo plot clean open collabs graphs

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sections/2-preliminaries.tex <==
% !TEX root = ../paper.tex

%\subsection{Databases and SQL Queries}

A \textit{relational database} is a set of relations (\textit{i.e., tables}), and a \textit{relation} is a bag or set of tuples (\textit{i.e., rows}) where a tuple is a structured data item. The structure is defined with attributes (\textit{i.e., columns}) and the types of the attributes. The difference between a bag and a set is that bag semantics allow duplicate records whereas set semantics enforce uniqueness.

%Relational Database Management Systems (RDMS) ensure result accuracy while providing efficiency for joining combination of multiple resources.
%The most important principle in these systems is that a query simply must not return a wrong result.

\textit{Structured Query Language (SQL)} is a declarative language that is designed for managing, manipulating, and retrieving from relational databases.
Other than schema manipulation and data access control operations, SQL queries mainly perform 4 different operations: (1) insert, (2) update, (3) delete, and (4) select. The basic structure of these operations are given respectively:

{\footnotesize
\begin{verbatim}
(1) INSERT INTO table (column1, column2, ...)
               VALUES (value1, value2, ...);
(2) UPDATE table
    SET column1 = integer|decimal|string|...
    WHERE column2 = integer|decimal|string|...
(3) DELETE FROM table
    WHERE column1 = integer|decimal|string|...
(4) SELECT [aggregation] column1, column2, ...
    FROM table1, table2
    [WHERE table1.column1 = table2.column3]
    [ORDER BY column1] [GROUP BY column1]
    [LIMIT integer]
\end{verbatim}
}

where the brackets show optional query items. As can be implied from these basic structures, queries that perform similar tasks usually have analogous structures, or at least share some attributes. 

SQL query statements are constructed from \textit{clauses}. Every line of the query structures given above constitutes a clause. As an example let's take the following query:

{\footnotesize
\begin{verbatim}
(1) SELECT u.username, u.yearenrolled
(2) FROM user u, accounts a
(3) WHERE u.id = a.userid AND a.balance > 1000
(4) GROUP BY u.yearenrolled
(5) ORDER BY u.yearenrolled
\end{verbatim}
}

Line 1 consists of the \texttt{SELECT} keyword, and the \textit{projection} items. Line 2 has the \texttt{FROM} clause which lists the tables the query is going to use. Line 3 is named the \texttt{WHERE} clause. Where clause contains \textit{selection} and \textit{join} expressions. \texttt{u.id = a.userid} expression is a join expression, and \texttt{a.balance > 1000} is a selection expression. Line 4 and 5 include the \textit{group-by} and \textit{order-by} items, respectively.

%\subsection{Database Security}
%\note{This section is here to emphasize the security research on databases right now is focusing on other issues, but our topic needs addressing, too.}

%The current research on database security focuses on different security aspects. 
%For instance, our framework can detect deviations from original behavior, but it cannot be used to detect the integrity of an outsourced database, or it cannot detect if an adversary takes a snapshot of the database server.
%However, the system proposed in this paper can be supported with, and integrated into the following database security measures.

%\tinysection{SQL injection prevention} If an application is vulnerable to the SQL Command Injection Attacks, the adversary can gain unauthorized access to the data that they normally are not authorized to access. One approach to overcome these attacks is to randomize the keywords in the SQL preprogrammed query~\cite{boyd2004sqlrand} while the other approach is to use benign candidate inputs to mine programmer intentions~\cite{bandhakavi2007candid}.

%\tinysection{Outsourced database integrity} Nowadays, many organizations prefer outsourcing the management of their systems and databases in order to reduce their costs.
%However, in this case, the outsourced database is accessible to the outsourced company systems and personnel which raises concerns on the query result trustworthiness.
%The current research focuses on interactive proofs and authenticated datastructures~\cite{zhang2015integridb, zhang2017vsql}.

%\tinysection{Encrypted databases} If intruders can infiltrate into the organization network, they can take a snapshot of the database systems. This line of research focuses on running SQL queries over encrypted data against data leakage~\cite{popa2011cryptdb, tu2013processing}, hence even if a snapshot attack is successful, the data stolen would be encrypted.

%Our proposed framework can be added as an observer to the SQL query parser of any relational DBMS to capture the issued query, regardless of if the DBMS implements any of the database security measures mentioned above as an additional defense mechanism.

==> sections/6-conclusion.tex <==
% !TEX root = ../paper.tex
The focus of this paper was to highlight a class of vulnerabilities that can lead to data leakage from the database system, and to present a framework for creating user behavior profiles considering the temporal behavior drift to be used in detecting attacks exploiting them. We first provided a user behavior model for data leakage prevention. We argued that without considering the constant change in people's behaviors and habits, it is impossible for the defense systems to adapt to the new changes. This would result in the need for retraining of the user models for the system. In our experiments, we used real world query workloads and applied two different red teaming approaches: (1) simulated attack workloads, and (2) injection of benign real world workloads of other users.
%We evaluated our system with and without temporal behavior drift model in detecting these injections. For both approaches, the TPRs consistently remained comparable. However, FPR comparison revealed that temporal behavior drift model remarkably reduced the FPR, hence validated our assumptions.

The model we described in this paper constitutes the first steps of building a temporal behavior drift prediction model. Concretely, we plan to extend our work in several directions: First, we will analyze other regression models, and test their effect on the performance of the system. Second, we incorporate a prediction model both for security applications, and performance optimization of database systems. Lastly, we will develop a production ready package to be integrated to apps and Android OS. %collect data in real world organizations, and test the system on site to eliminate privacy concerns.

==> sections/graph.tex <==
\todo{ROC graphs}

\begin{figure}[h!]
	\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
		\caption{Facebook}
        \label{fig:roccurve:Facebook}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
        \caption{Google+}
        \label{fig:roccurve:GooglePlus}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
        \caption{Hangouts}
        \label{fig:roccurve:Hangouts}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
        \caption{Google Play Services}
        \label{fig:roccurve:GooglePlayServices}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
        \caption{Media Storage}
        \label{fig:roccurve:MediaStorage}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}%{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/roccurve.png}
        \caption{Complete Workload}
        \label{fig:roccurve:CompleteWorkload}
    \end{subfigure}
    \caption{ROC Graph for different Android applications}
    \label{fig:roccurve}
\end{figure}


http://gim.unmc.edu/dxtests/roc2.htm

\begin{table}[]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{llllll}
                                                               & \begin{tabular}[c]{@{}l@{}}Number\\ of Attacks\end{tabular} & \begin{tabular}[c]{@{}l@{}}True Positive\\ Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}False Positive\\ Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}True Positive\\ Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}False Positive\\ Rate\end{tabular} \\
Facebook                                                       & 309                                                         & 89.64\%                                                      & 13.59\%                                                       & 92.55\%                                                      & 20.38\%                                                       \\
Google+                                                        & 2120                                                        & 89.76\%                                                      & 10.37\%                                                       & 89.95\%                                                      & 16.03\%                                                       \\
Hangouts                                                       & 2390                                                        & 84.18\%                                                      & 9.62\%                                                        & 83.72\%                                                      & 52.08\%                                                       \\
\begin{tabular}[c]{@{}l@{}}Google Play\\ Services\end{tabular} & 2310                                                        & 90.08\%                                                      & 10.77\%                                                       & 90.86\%                                                      & 15.93\%                                                       \\
Media Storage                                                  & 2028                                                        & 91.46\%                                                      & 9.91\%                                                        & 88.85\%                                                      & 20.46\%                                                      
\end{tabular}
\end{table}


\begin{figure*}[h]
\captionsetup[subfigure]{justification=centering}
\centering
%\begin{tabular}{c c}
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=.6\textwidth]{graphs/APK}
  \caption{APK file structure}
  \label{fig:sub1}
\end{subfigure}
%& \multirow{2}{*}{
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=.6\textwidth]{graphs/DEX}
  \caption{DEX file structure}
  \label{fig:sub2}
\end{subfigure}
%}
% \\
~
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=.6\textwidth]{graphs/Malicious}
  \caption{APK+DEX}
  \label{fig:sub3}
\end{subfigure}
%\end{tabular}
\caption{Embedding DEX into APK files}
\label{fig:janus}
\end{figure*}
